Joint estimation of insurance loss development factors using Bayesian hidden Markov models

Loss development modelling is the actuarial practice of predicting the total 'ultimate' losses incurred on a set of policies once all claims are reported and settled. This poses a challenging prediction task as losses frequently take years to fully emerge from reported claims, and not all claims might yet be reported. Loss development models frequently estimate a set of 'link ratios' from insurance loss triangles, which are multiplicative factors transforming losses at one time point to ultimate. However, link ratios estimated using classical methods typically underestimate ultimate losses and cannot be extrapolated outside the domains of the triangle, requiring extension by 'tail factors' from another model. Although flexible, this two-step process relies on subjective decision points that might bias inference. Methods that jointly estimate 'body' link ratios and smooth tail factors offer an attractive alternative. This paper proposes a novel application of Bayesian hidden Markov models to loss development modelling, where discrete, latent states representing body and tail processes are automatically learned from the data. The hidden Markov development model is found to perform comparably to, and frequently better than, the two-step approach, as well as a latent change-point model, on numerical examples and industry datasets.

==> src/backtest.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{\figures/atas.png}
    \caption{
        The empirical link ratios by line of business in
        the \cite{meyers2015} dataset.
        Points indicate the mean across triangles,
        and vertical line segments show 2 standard
        deviations.
    }
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{\figures/scores.png}
    \caption{
        The ELPD (left column) and RMSE (in dollars; right column)
        for each of the four models and line of business
        in the industry backtest. The ELPD values are remove
		any cell's predictions that have a log likelihood value
		$\leq -100$, to not bias the results unfairly towards poorly
		performing predictions.
    }
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale=0.5]{\figures/calibration.png}
    \caption{
        Percentiles of the true values on the posterior distributions
        for each model and line of business in the backtest.
    }
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{\figures/z_stars.png}
    \caption{
        The average probability of being in the tail process
        for each hidden Markov model parameterization
        and line of business in the backtest data.
        Probabilities $\leq 0.5$ are coloured
        in blue whereas probabilities $> 0.5$
        are coloured in green. Faded squares
        indicating smaller probabilities of being
        in body and tail processes, respectively.
    }
\end{figure}

